Generalizing Denoising to Non-Equilibrium Structures Improves Equivariant Force Fields

Understanding the interactions of atoms such as forces in 3D atomistic systems is fundamental to many applications like molecular dynamics and catalyst design. However, simulating these interactions requires compute-intensive ab initio calculations and thus results in limited data for training neural networks. In this paper, we propose to use denoising non-equilibrium structures (DeNS) as an auxiliary task to better leverage training data and improve performance. For training with DeNS, we first corrupt a 3D structure by adding noise to its 3D coordinates and then predict the noise. Different from previous works on denoising, which are limited to equilibrium structures, the proposed method generalizes denoising to a much larger set of non-equilibrium structures. The main difference is that a non-equilibrium structure does not correspond to local energy minima and has non-zero forces, and therefore it can have many possible atomic positions compared to an equilibrium structure. This makes denoising non-equilibrium structures an ill-posed problem since the target of denoising is not uniquely defined. Our key insight is to additionally encode the forces of the original non-equilibrium structure to specify which non-equilibrium structure we are denoising. Concretely, given a corrupted non-equilibrium structure and the forces of the original one, we predict the non-equilibrium structure satisfying the input forces instead of any arbitrary structures. Since DeNS requires encoding forces, DeNS favors equivariant networks, which can easily incorporate forces and other higher-order tensors in node embeddings. We study the effectiveness of training equivariant networks with DeNS on OC20, OC22 and MD17 datasets and demonstrate that DeNS can achieve new state-of-the-art results on OC20 and OC22 and significantly improve training efficiency on MD17.

==> content/5_4_ablation_study.tex <==
\vspace{-2mm}

\begin{table}[t]
\centering
\scalebox{0.6}{

\begin{tabular}{cccclcccccccccc}
\toprule[1.2pt]
& \multicolumn{3}{c}{Methods} & & \\
\cmidrule[0.6pt]{2-4}
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-linear \\ message passing\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MLP \\ attention\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dot product \\ attention\end{tabular}} &  Task & $\alpha$ & $\Delta \varepsilon$ & $\varepsilon_{\text{HOMO}}$ & $\varepsilon_{\text{LUMO}}$ & $\mu$ & $C_{\nu}$ & & Training time & Number of \\
%Index & & & & Unit & bohr$^3$ & meV & meV & meV & D & cal/mol K & & (minutes/epoch) & parameters \\
Index & & & & Unit & $a_0^3$ & meV & meV & meV & D & cal/mol K & & (minutes/epoch) & parameters \\
\midrule[1.2pt]

1 & \ding{51} & \ding{51} &  & & .046 & 30 & 15 & 14 & .011 & .023 & & 12.1 & 3.53M \\
2 & & \ding{51} &   & & .051 & 32 & 16 & 16 & .013 & .025 & & 7.2 & 3.01M \\
3 & & & \ding{51} & & .053 & 32 & 17 & 16 & .013 & .025 & & 7.8 & 3.35M \\
%4 & & \ding{51} &  &  & & .060 &  & 18 & 17 & .016 &  \\

\bottomrule[1.2pt]

\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{Ablation study results on QM9.}}
\vspace{-3.25mm}
\label{tab:qm9_ablation}
\end{table}


\begin{table}[t]
\begin{adjustwidth}{-5 cm}{-5 cm}
\centering
\scalebox{0.6}{

\begin{tabular}{cccccccccccccccccc}
\toprule[1.2pt]
& \multicolumn{3}{c}{Methods} & & \multicolumn{5}{c}{Energy MAE (eV) $\downarrow$} & & \multicolumn{5}{c}{EwT (\%) $\uparrow$} \\
\cmidrule[0.6pt]{2-4}
\cmidrule[0.6pt]{6-10}
\cmidrule[0.6pt]{12-16}
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-linear \\ message passing\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MLP \\ attention\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dot product \\ attention\end{tabular}} & & & & & & & & & & & & & Training time & Number of \\

Index & & & &  & ID & OOD Ads & OOD Cat & OOD Both & Average & & ID & OOD Ads & OOD Cat & OOD Both & Average & (minutes/epoch) & parameters \\
\midrule[1.2pt]

1 & \ding{51} & \ding{51} &  & & 0.5088 & 0.6271 & 0.5051 & 0.5545 &  0.5489  & & 4.88 & 2.93 & 4.92 & 2.98 & 3.93 & 130.8 & 9.12M \\
2 & & \ding{51} &   & & 0.5168 & 0.6308 & 0.5088 & 0.5657 & 0.5555 &  & 4.59 & 2.82 & 4.79 & 3.02 & 3.81 & 91.2 & 7.84M \\
3 & & & \ding{51}  & & 0.5386 & 0.6382 & 0.5297 & 0.5692 & 0.5689 & & 4.37 & 2.60 & 4.36 & 2.86 & 3.55 & 99.3 & 8.72M \\
%4 & & \ding{51} &  &  & 0.5213 & 0.6268 & 0.5178 & 0.5621 & 0.5579\\

%\bottomrule[1.2pt]
%\bottomrule[1.2pt]
%\vspace{-1mm}
%\\
%\toprule[1.2pt]

%%%\midrule[1.2pt]
%%%& \multicolumn{3}{c}{Methods} & & \multicolumn{5}{c}{EwT (\%) $\uparrow$} \\
%%%\cmidrule[0.6pt]{2-4}
%%%\cmidrule[0.6pt]{6-10}
%%%& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-linear \\ message passing\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MLP \\ attention\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Dot product \\ attention\end{tabular}} &  \\

%%%Index & & & & & ID & OOD Ads & OOD Cat & OOD Both & Average \\
%%%\midrule[1.2pt]

%%%1 & \ding{51} & \ding{51} & & & 4.88 & 2.93 & 4.92 & 2.98 & 3.93 \\
%%%2 & & \ding{51} &   &  & 4.59 & 2.82 & 4.79 & 3.02 & 3.81  \\
%%%3 & & & \ding{51} & & 4.37 & 2.60 & 4.36 & 2.86 & 3.55 \\
%4 & & \ding{51} &  &  & 4.37 & 2.80 & 4.40 & 2.98 & 3.64 \\

\bottomrule[1.2pt]

\end{tabular}
}

\vspace{-3mm}
\end{adjustwidth}
\caption{\textbf{Ablation study results on OC20 IS2RE validation set.}
%\note{Dot product attention uses smaller learning rate $1.5 \times 10^{-3}$.}
}
\vspace{-6.75mm}
\label{tab:oc20_ablation}
\end{table}



\vspace{-2.25mm}
\subsection{Ablation Study}
\vspace{-2.5mm} 
\label{subsec:ablation_study}

We conduct ablation studies \revision{to show that Equiformer with dot product attention and linear message passing has already achieved strong empirical results and demonstrate} the improvement brought by MLP attention and non-linear messages in the proposed equivariant graph attention.
%We modify dot product (DP) attention~\citep{transformer, se3_transformer} so that it only differs from MLP attention in how attention weights $a_{ij}$ are generated from $f_{ij}$.
\revision{Dot product (DP) attention only differs from MLP attention in how attention weights $a_{ij}$ are generated from $f_{ij}$.}
%%%Please refer to Sec.~\ref{appendix:subsec:dot_product_attention} in appendix for details on DP attention.
Please refer to Sec.~\ref{appendix:subsec:dot_product_attention} in appendix for further details.
For experiments on QM9 and OC20, unless otherwise stated, we follow the hyper-parameters used in previous experiments. 
%\revision{Please refer to Sec.~\ref{appendix:subsec:qm9_training_details} and Sec.~\ref{appendix:subsec:oc20_training_details} for training time of different models.}

\vspace{-3.25mm}
\paragraph{Result on QM9.}
The comparison is summarized in Table~\ref{tab:qm9_ablation}.
\revision{Compared with models in Table~\ref{tab:qm9_result}, Equiformer with dot product attention and linear message passing (Index 3) achieves competitve results.}
%Non-linear messages improve upon linear messages when MLP attention is used.
Non-linear messages improve upon linear messages when MLP attention is used while non-linear messages increase the number of tensor product operations in each block from $1$ to $2$ and thus inevitably increase training time.
%%%Similar to what is reported by GATv2~\cite{gatv2}, the improvement of replacing DP attention with MLP attention is not very significant.
%%%\todo{On the other hand, the improvement of replacing DP attention with MLP attention is not very significant.}
On the other hand, MLP attention achieves similar results to DP  attention.
We conjecture that DP attention with linear operations is expressive enough to capture common attention patterns as the numbers of nighboring nodes and atom species are much smaller than those in OC20.
However, MLP attention is roughly $8\%$ faster as it directly generates scalar features and attention weights from $f_{ij}$ instead of producing additional key and query irreps features for attention weights.

\vspace{-3.25mm}
\paragraph{Result on OC20.}
%%%We consider the setting of training without IS2RS auxiliary task and use a smaller learning rate $1.5 \times 10 ^{-4}$ for DP attention as this improves the performance.
We consider the setting of training without auxiliary task and summarize the comparison in Table~\ref{tab:oc20_ablation}.
%%%We summarize the comparison in Table~\ref{tab:oc20_ablation}.
\revision{Compared with models in Table~\ref{tab:is2re_validation}, Equiformer with dot product attention and linear message passing (Index 3) has already outperformed all previous models.}
Non-linear messages consistently improve upon linear messages.
In contrast to the results on QM9, MLP attention achieves better performance than DP attention and is $8\%$ faster.
We surmise this is because OC20 contains larger atomistic graphs with more diverse atom species and therefore requires more expressive attention mechanisms.
Note that Equiformer can potentially improve upon previous equivariant Transformers~\citep{se3_transformer, torchmd_net, eqgat} since they use less expressive attention mechanisms similar to Index 3 in Table~\ref{tab:oc20_ablation}.

==> content/7_checklist.tex <==

\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code related to experiments on QM9 in supplementary. Code reproducing all experiments will be available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{As each experiment takes much time, we are not able to run several times. However, the proposed method improves upon previous works by a clear margin, and therefore the improvement is not within noise ranges.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> content/8_2_details_of_architecture.tex <==
\section{Details of Architecture}
\label{appendix:sec:details_of_architecture}

In this section, we define architectural hyper-parameters like maximum degrees and numbers of channels  in certain layers in EquiformerV2, which are used to specify the detailed architectures in Sec.~\ref{appendix:subsec:training_details}.
Besides, we note that eSCN~\cite{escn} and this work mainly consider $SE(3)$-equivariance.


We denote embedding dimensions as $d_{embed}$, which defines the dimensions of most irreps features.
Specifically, the output irreps features of all modules except the output head in Figure~\ref{fig:equiformer_v2}a have dimension $d_{embed}$.
%Specifically, the output irreps features of all modules except the output head in Figure {\color{crimson}1}a have dimension $d_{embed}$.
For separable $S^2$ activation as illustrated in Figure~\ref{fig:activation}c, we denote the resolution of point samples on a sphere as $R$, which can depend on maximum degree $L_{max}$, and denote the unconstrained functions after projecting to point samples as $F$.
%For separable $S^2$ activation as illustrated in Figure {\color{crimson}2}c, we denote the resolution of point samples on a sphere as $R$, which can depend on maximum degree $L_{max}$, and denote the unconstrained functions after projecting to point samples as $F$.


For equivariant graph attention in Figure~\ref{fig:equiformer_v2}b, the input irreps features $x_i$ and $x_j$ have dimension $d_{embed}$.
%For equivariant graph attention in Figure {\color{crimson}1}b, the input irreps features $x_i$ and $x_j$ have dimension $d_{embed}$.
The dimension of the irreps feature $f_{ij}^{(L)}$ is denoted as $d_{attn\_hidden}$.
Equivariant graph attention can have $h$ parallel attention functions.
For each attention function, we denote the dimension of the scalar feature $f_{ij}^{(0)}$ as $d_{attn\_alpha}$ and denote the dimension of the value vector, which is in the form of irreps features, as $d_{attn\_value}$.
For the separable $S^2$ activation used in equivariant graph attention, the resolution of point samples is $R$, and we use a single SiLU activation for $F$.
We share the layer normalization in attention re-normalization across all $h$ attention functions but have different $h$ linear layers after that.
The last linear layer projects the dimension back to $d_{embed}$.
The two intermediate $SO(2)$ linear layers operate with maximum degree $L_{max}$ and maximum order $M_{max}$.


For feed forward networks (FFNs) in Figure~\ref{fig:equiformer_v2}d, we denote the dimension of the output irreps features of the first linear layer as $d_{ffn}$.
%For feed forward networks (FFNs) in Figure {\color{crimson}1}d, we denote the dimension of the output irreps features of the first linear layer as $d_{ffn}$.
%For the separable $S^2$ activation in Figure~\ref{fig:equiformer_v2}d, the resolution of point samples is $R$, and $F$ consists of a two-layer MLP, with each linear layer followed by SiLU, and a final linear layer.
For the separable $S^2$ activation used in FFNs, the resolution of point samples is $R$, and $F$ consists of a two-layer MLP, with each linear layer followed by SiLU, and a final linear layer.
The linear layers have the same number of channels as $d_{ffn}$.
%The FFN in the last Transformer block has output dimension $d_{feature}$, and we set $d_{ffn}$ of the last FFN, which is followed by output head, to be $d_{feature}$ as well.
%Thus, two hyper-parameters $d_{ffn}$ and $d_{feature}$ are used to specify architectures of FFNs and the output dimension after Transformer blocks.

For radial functions, we denote the dimension of hidden scalar features as $d_{edge}$.
For experiments on OC20, same as eSCN~\cite{escn}, we use Gaussian radial basis to represent relative distances and additionally embed the atomic numbers at source nodes and target nodes with two scalar features of dimension $d_{edge}$.
The radial basis and the two embeddings of atomic numbers are fed to the radial function to generate edge distance embeddings.

%Irreps features contain channels of vectors with degrees up to $L_{max}$.
%We denote $C_L$ type-$L$ vectors as $(C_L, L)$ and $C_{(L, p)}$ type-$(L, p)$ vectors as $(C_{(L, p)}, L, p)$ and use brackets to represent concatenations of vectors.
%For example, the dimension of irreps features containing $256$ type-$0$ vectors and $128$ type-$1$ vectors can be represented as $[(256, 0), (128, 1)]$.
%We can extend this to include inversion by introducing parity $p$ and using $(C_{(L, p)}, L, p)$.

The maximum degree of irreps features is denoted as $L_{max}$.
All irreps features have degrees from $0$ to $L_{max}$ and have $C$ channels for each degree.
We denote the dimension as $(L_{max}, C)$.
For example, irreps feature $x_{irreps}$ of dimension $(6, 128)$ has maximum degree $6$ and $128$ channels for each degree.
The dimension of scalar feature $x_{scalar}$ can be expressed as $(0, C_{scalar})$.

Following Equiformer~\cite{equiformer}, we apply dropout~\cite{dropout} to attention weights and stochastic depth~\cite{drop_path} to outputs of equivariant graph attention and feed forward networks.
However, we do not apply dropout or stochastic depth to the output head.





==> content/8_3_details_of_experiments_on_oc20.tex <==
\section{Details of Experiments on OC20}
\label{appendix:sec:details_of_experiments_on_oc20}





\begin{comment}
\begin{enumerate}
    \item \todo{Training and architectural hyper-parameters.}
    \begin{enumerate}
        \item \todo{S2EF-2M.}
        \item \todo{S2EF-All.}
    \end{enumerate}

    \item \todo{Training time/inference time and number of parameters.}
    \begin{enumerate}
        \item \todo{S2EF-2M.}
        \begin{enumerate}
            \item \todo{Architectural improvements.}
            \item \todo{Scaling of Parameters.}
            \item \todo{Speed-Accuracy Trade-offs.}
        \end{enumerate}
        \item \todo{S2EF-All.}
    \end{enumerate}

    \item \todo{Details of running relaxations.}

    \item \todo{Details of running AdsorbML.}
        \begin{enumerate}
            \item \todo{Runtime (in terms of GPU-hours and CPU-hours) for each $k$ and each model if possible.}
        \end{enumerate}
\end{enumerate}
\end{comment}


\begin{table}[t]
\centering
\scalebox{0.65}{
\begin{tabular}{llll}
%\cline{7-11}
%\toprule[1.2pt]
& \multicolumn{1}{c}{Base model setting on} & \multicolumn{1}{c}{EquiformerV2 ($31$M) on} & \multicolumn{1}{c}{EquiformerV2 ($153$M) on} \\
Hyper-parameters & \multicolumn{1}{c}{S2EF-2M} & \multicolumn{1}{c}{S2EF-All+MD} & \multicolumn{1}{c}{S2EF-All/S2EF-All+MD} \\
\midrule
Optimizer & AdamW & AdamW & AdamW \\
%Learning rate scheduling & Cosine learning rate with linear warmup \\
Learning rate scheduling & Cosine learning rate with & Cosine learning rate with & Cosine learning rate with \\
& linear warmup & linear warmup & linear warmup \\
Warmup epochs & $0.1$ & $0.01$ & $0.01$ \\
Maximum learning rate & $2 \times 10 ^{-4}$ & $4 \times 10 ^{-4}$ & $4 \times 10 ^{-4}$ \\
Batch size & $64$ & $512$ & $256$ for S2EF-All, \\
& & & $512$ for S2EF-All+MD \\
Number of epochs & $12$ & $3$ & $1$ \\
Weight decay & $1 \times 10 ^{-3}$ & $1 \times 10 ^{-3}$ & $1 \times 10 ^{-3}$\\
Dropout rate & $0.1$ & $0.1$ & $0.1$ \\
Stochastic depth & $0.05$ & $0.1$ & $0.1$ \\
Energy coefficient $\lambda_{E}$ & $2$ & $4$ & $2$ for S2EF-All, \\
& & & $2, 4$ for S2EF-All+MD \\
Force coefficient $\lambda_{F}$ & $100$ & $100$ & $100$ \\
Gradient clipping norm threshold & $100$ & $100$ & $100$ \\
Model EMA decay & $0.999$ & $0.999$ & $0.999$ \\
%\midrule[0.6pt]
Cutoff radius ($\angstrom$) & $12$ & $12$ & $12$ \\
Maximum number of neighbors & $20$ & $20$ & $20$ \\
Number of radial basis & $600$ & $600$ & $600$ \\
Dimension of hidden scalar features in radial functions $d_{edge}$ & $(0, 128)$ & $(0, 128)$ & $(0, 128)$ \\
%Hidden size of radial function & $64$ \\
%Number of hidden layers in radial function & $2$ \\

%\midrule[0.6pt]

%\multicolumn{2}{c}{Equiformer} \\
%\\
Maximum degree $L_{max}$ & $6$ & $4$ & $6$ \\
Maximum order $M_{max}$ & $2$ & $2$ & $3$\\
Number of Transformer blocks & $12$ & $8$ & $20$ \\
Embedding dimension $d_{embed}$ & $(6, 128)$ & $(4, 128)$ & $(6, 128)$ \\
%Spherical harmonics embedding dimension $d_{sh}$ & $[(1, 0), (1, 1)]$ \\
$f_{ij}^{(L)}$ dimension $d_{attn\_hidden}$ & $(6, 64)$ & $(4, 64)$ & $(6, 64)$ \\
Number of attention heads $h$ & $8$ & $8$ & $8$ \\
$f_{ij}^{(0)}$ dimension $d_{attn\_alpha}$ & $(0, 64)$ & $(0, 64)$ & $(0, 64)$ \\
Value dimension $d_{attn\_value}$ & $(6, 16)$ & $(4, 16)$ & $(6, 16)$\\
%Attention head dimension $d_{head}$ & $[(32, 0), (16, 1)]$\\
Hidden dimension in feed forward networks $d_{ffn}$ & $(6, 128)$ & $(4, 128)$ & $(6, 128)$ \\
Resolution of point samples $R$ & $18$ & $18$ & $18$ \\

%\midrule[0.6pt]

%\multicolumn{2}{c}{$E(3)$-Equiformer} \\
%\\
%Number of Transformer blocks & $6$ \\
%Embedding dimension $d_{embed}$ & $[(256, 0, e), (64, 0, o), (64, 1, e), (64, 1, o)]$ \\
%Spherical harmonics embedding dimension $d_{sh}$ & $[(1, 0, e), (1, 1, o)]$ \\
%Number of attention heads $h$ & $8$ \\
%Attention head dimension $d_{head}$ & $[(32, 0, e), (8, 0, o), (8, 1, e), (8, 1, o)]$ \\
%Hidden dimension in feed forward networks $d_{ffn}$ & $[(768, 0, e), (192, 0, o), (192, 1, e), (192, 1, o)]$ \\
%Output feature dimension $d_{feature}$ & $[(512, 0, e)]$\\

%\bottomrule[1.2pt]
\end{tabular}
}
\vspace{2mm}
\caption{Hyper-parameters for the base model setting on OC20 S2EF-2M dataset and the main results on OC20 S2EF-All and S2EF-All+MD datasets.
}
\label{appendix:tab:oc20_s2ef_hyperparameters}
\end{table}



\begin{table}[t]
\begin{adjustwidth}{-5cm}{-5cm}
\centering
\scalebox{0.55}{
\begin{tabular}{lccccccccc}
& Attention & & & & & Number of & Training time & Inference speed & Number of \\
Training set & re-normalization & Activation & Normalization & $L_{max}$ & $M_{max}$ & Transformer blocks & (GPU-hours) & (Samples / GPU sec.) & parameters \\
\shline
\multirow{10}{*}{S2EF-2M} & \xmark & Gate & LN & $6$ & $2$ & $12$ & $965$ & $19.06$ & $91.06$M \\
& \cmark & Gate & LN & 6 & 2 & 12 & $998$ & $19.07$ & $91.06$M \\
& \cmark & $S^{2}$ & LN & $6$ & $2$ & $12$ & $1476$ & $12.80$ & $81.46$M \\
& \cmark & Sep. $S^{2}$ & LN & $6$ & $2$ & $12$ & $1505$ & $12.51$ & $83.16$M \\
& \cmark & Sep. $S^{2}$ & SLN & $6$ & $2$ & $12$ & $1412$ & $13.22$ & $83.16$M \\

& \cmark & Sep. $S^{2}$ & SLN & $4$ & $2$ & $12$ & $965$ & $19.86$ & $44.83$M \\
& \cmark & Sep. $S^{2}$ & SLN & $8$ & $2$ & $12$ & $2709$ & $7.86$ & $134.28$M \\
& \cmark & Sep. $S^{2}$ & SLN & $6$ & $3$ & $12$ & $1623$ & $11.92$ & $95.11$M \\
& \cmark & Sep. $S^{2}$ & SLN & $6$ & $4$ & $12$ & $2706$ & $7.98$ & $102.14$M \\
& \cmark & Sep. $S^{2}$ & SLN & $6$ & $6$ & $12$ & $3052$ & $7.13$ & $106.63$M \\


\midrule
S2EF-All & \cmark & Sep. $S^{2}$ & SLN & $6$ & $3$ & $20$ & $20499$ & $6.08$ & $153.60$M \\

\midrule
S2EF-All+MD ($\lambda_{E} = 2$)& \cmark & Sep. $S^{2}$ & SLN & $6$ & $3$ & $20$ & $32834$ & $6.08$ & $153.60$M \\

\midrule
S2EF-All+MD ($\lambda_{E} = 4$)& \cmark & Sep. $S^{2}$ & SLN & $4$ & $2$ & $8$ & $16931$ & $29.21$ & $31.06$M \\
S2EF-All+MD ($\lambda_{E} = 4$)& \cmark & Sep. $S^{2}$ & SLN & $6$ & $3$ & $20$ & $37692$ & $6.08$ & $153.60$M \\
\end{tabular}
}
\vspace{2mm}
\end{adjustwidth}
\caption{Training time, inference speed and numbers of parameters of different models trained on OC20 S2EF-2M, S2EF-All and S2EF-All+MD datasets.
All numbers are measured on V100 GPUs with 32GB.
}
\label{appendix:tab:training_time_inference_speed_and_numbers_of_parameters}
\end{table}


\subsection{Training Details}
\label{appendix:subsec:training_details}

\paragraph{Hyper-Parameters.}
We summarize the hyper-parameters for the base model setting on OC20 S2EF-2M dataset and the main results on OC20 S2EF-All and S2EF-All+MD datasets in Table~\ref{appendix:tab:oc20_s2ef_hyperparameters}.
%For the ablation studies on OC20 S2EF-2M dataset, when trained for $20$ or $30$ epochs as in Table {\color{crimson}1b}, we increase the learning rate from $2 \times 10^{-4}$ to $4 \times 10^{-4}$.
For the ablation studies on OC20 S2EF-2M dataset, when trained for $20$ or $30$ epochs as in~\tableref{tab:training_epochs}, we increase the learning rate from $2 \times 10^{-4}$ to $4 \times 10^{-4}$.
%When using $L_{max} = 8$ as in Table {\color{crimson}1c}, we increase the resolution of point samples $R$ from $18$ to $20$.
When using $L_{max} = 8$ as in~\tableref{tab:l_degrees}, we increase the resolution of point samples $R$ from $18$ to $20$.
%We vary $L_{max}$ and the widths for speed-accuracy trade-offs in Figure {\color{crimson}4}.
We vary $L_{max}$ and the widths for speed-accuracy trade-offs in Figure~\ref{fig:combined_train_test_throughput}.
Specifically, we first decrease $L_{max}$ from $6$ to $4$.
Then, we multiply $h$ and the number of channels of $(d_{embed}, d_{attn\_hidden}, d_{ffn})$ by $0.75$ and $0.5$.
We train all models for $30$ epochs.
The same strategy to scale down eSCN models is adopted for fair comparisons.


\paragraph{Training Time, Inference Speed and Numbers of Parameters.}
Table~\ref{appendix:tab:training_time_inference_speed_and_numbers_of_parameters} summarizes the training time, inference speed and numbers of parameters of models in Tables~\ref{tab:ablations} (row 1, 2, 3, 4, 5),~\ref{tab:l_degrees},~\ref{tab:m_orders} and~\ref{tab:oc20_all_results}.
%Table~\ref{appendix:tab:training_time_inference_speed_and_numbers_of_parameters} summarizes the training time, inference speed and numbers of parameters of models in Tables {\color{crimson}1a} (row 1, 2, 3, 4, 5), {\color{crimson}1c}, {\color{crimson}1d} and {\color{crimson}2}.
%For S2EF-2M dataset, models are trained for $12$ epochs.
V100 GPUs with 32GB are used to train all models.
We use $16$ GPUs to train each individual model on S2EF-2M dataset, $64$ GPUs for S2EF-All, $64$ GPUs for EquiformerV2 ($31$M) on S2EF-All+MD, and $128$ GPUs for EquiformerV2 ($153$M) on S2EF-All+MD.



\subsection{Details of Running Relaxations}
\label{appendix:subsec:details_of_running_relaxations}
%A structural relaxation is a local optimization where atom positions are iteratively updated based on the forces to minimize the energy.
A structural relaxation is a local optimization where atom positions are iteratively updated based on forces to minimize the energy of the structure.
%We performed all of our ML relaxations using the LBFGS optimizer (quasi-Newton) implemented in the Open Catalyst Github repository, full optimizer settings are listed below.
We perform ML relaxations using the LBFGS optimizer (quasi-Newton) implemented in the Open Catalyst Github repository~\cite{oc20}.
%All OC20 optimizations were allowed to run for up to 200 steps or until $F_{max} \leq 0.02$ eV/\angstrom, whereas AdsorbML relaxations were allowed to run for 300 steps or until $F_{max} \leq 0.02$ eV/\angstrom. These settings were chosen to be consistent with prior work.
The structural relaxations for OC20 IS2RE and IS2RS tasks are allowed to run for $200$ steps or until the maximum predicted force per atom $F_{max} \leq 0.02$ eV/\angstrom, and the relaxations for AdsorbML are allowed to run for $300$ steps or until $F_{max} \leq 0.02$ eV/\angstrom.
These settings are chosen to be consistent with prior works.
\revision{We run relaxations on V100 GPUs with 32GB.}
\revision{The computational cost of running relaxations with EquiformerV2 ($153$M) for OC20 IS2RE and IS2RS tasks is $1011$ GPU-hours, and that of running ML relaxations for AdsorbML is $1075$ GPU-hours.}
%\ad{The time for running relaxations with EquiformerV2 ($31$M) is 240 GPU-hours for IS2RE and IS2RS, and 298 GPU-hours for AdsorbML.}
The time for running relaxations with EquiformerV2 ($31$M) is 240 GPU-hours for OC20 IS2RE and IS2RS and 298 GPU-hours for AdsorbML.




\subsection{Details of AdsorbML}
\label{appendix:subsec:details_of_adsorbml}

%We ran the AdsorbML algorithm on the OC20-Dense dataset in accordance with the procedure laid out in the paper, which is summarized here:
We run the AdsorbML algorithm on the OC20-Dense dataset in accordance with the procedure laid out in the paper~\cite{adsorbml}, which is summarized here:

\begin{enumerate}
  %\item Run ML relaxations on all initial structures in OC20-Dense. There are around 1000 different adsorbate-surface combinations with $\sim$90 adsorbate placements per combination, so $\sim$90k in total.
  \item Run ML relaxations on all initial structures in the OC20-Dense dataset. There are around $1000$ different adsorbate-surface combinations with about $90$ adsorbate placements per combination, and therefore we have roughly $90$k structures in total.
  %\item Remove invalid relaxed structures based on the physical constraints and sort based on the lowest ML energy.
  \item Remove invalid ML relaxed structures based on physical constraints and rank the other ML relaxed structures in order of lowest to highest ML predicted energy.
  %\item Take the top 5 (lowest energy) ML relaxed structures for each system and run DFT single-points ($\sim$5000). DFT single-points calculations were run with VASP using the same functional RPBE and settings as the original AdsorbML experiments.
  \item Take the top $k$ ML relaxed structures with the lowest ML predicted energies for each adsorbate-surface combination and run DFT single-point calculations.
  The single-point calculations are performed on the ML relaxed structures to improve the energy predictions without running a full DFT relaxation and are run with VASP using the same setting as the original AdsorbML experiments.
  \revision{As shown in Table~\ref{tab:adsorbml}, we vary $k$ from $1$ to $5$.}
  %\revision{As shown in Table {\color{crimson}3}, we vary $k$ from $1$ to $5$.}
  %\todo{AdsorbML CPU-hours for DFT single-point calculations.}
  %The calculations are run with VASP using the same functional RPBE and settings as the original AdsorbML experiments.
  %\revision{The DFT single-point calculations are performed once for each relaxed structure and aim at providing a better energy measurement of the ML relaxed structures.}
  %\item Compute success and speedup metrics based on our lowest DFT single-point energy per system and the DFT labels provided with the dataset.
  \item Compute success and speedup metrics based on our lowest DFT single-point energy per adsorbate-surface combination and the DFT labels provided in the OC20-Dense dataset.
\end{enumerate}


We visualize some examples of relaxed structures from eSCN~\cite{escn}, EquiformerV2 and DFT in Figure~\ref{appendix:fig:relaxations_qualitative}.

%\newpage

\begin{figure}[t]
    \includegraphics[width=0.9\linewidth]{figures/relaxations_qualitative.jpg}
    \centering
    \vspace{1mm}
    \caption{Qualitative examples of the initial configuration of an adsorbate
    on a catalyst surface (column 1), and corresponding relaxed configurations
    obtained from eSCN~\cite{escn} (column 2), EquiformerV2 (column 3), and DFT
    (column 4). All examples are selected from the OC20-Dense dataset~\cite{adsorbml}.
    We show top-down views of each structure, with dashed lines showing the boundary of the unit cell repeating in the $x$ and $y$ directions.}
    \vspace{-4mm}
    \label{appendix:fig:relaxations_qualitative}
\end{figure}

==> content/8_4_broader_impacts.tex <==
\section{Broader Impacts}
\label{appendix:sec:broader_impacts}


==> content/8_5_limitations.tex <==
\section{Limitations}
\label{appendix:sec:limitations}


==> content/8_6_oc20.tex <==
\section{Details of Experiments on OC20}
\label{appendix:sec:oc20}


\subsection{Detailed Description of OC20 Dataset}
\label{appendix:subsec:oc20_dataset_details}
The dataset consists of larger atomic systems, each composed of a molecule called adsorbate placed on a slab called catalyst.
Each input contains more atoms and more diverse atom types than QM9 and MD17.
The average number of atoms in a system is more than 70, and there are over 50 atom species.
The goal is to understand interaction between adsorbates and catalysts through relaxation.
%Specifically, an adsorbate is first placed on top of a catalyst at heuristically determined locations in order to form initial structure (IS).
An adsorbate is first placed on top of a catalyst to form initial structure (IS).
The positions of atoms are updated with forces calculated by density function theory until the system is stable and becomes relaxed structure (RS).
The energy of RS, or relaxed energy (RE), is correlated with catalyst activity and therefore a metric for understanding their interaction.
We focus on the task of initial structure to relaxed energy (IS2RE), which predicts relaxed energy (RE) given an initial structure (IS).
%We focus on the task of initial structure to relaxed energy (IS2RE), which is to predict the energy of a relaxed structure (RS) given its initial structure (IS).
There are 460k, 100k and 100k structures in training, validation, and testing sets, respectively.
%%%Performance is measured in MAE and energy within threshold (EwT), the percentage in which predicted energy is within 0.02~eV of ground truth energy.
%%%In validation and testing sets, there are four sub-splits containing in-distribution adsorbates and catalysts (ID), out-of-distribution adsorbates (OOD-Ads), out-of-distribution catalysts (OOD-Cat), and out-of-distribution adsorbates and catalysts (OOD-Both).



\subsection{Training Details}
\label{appendix:subsec:oc20_training_details}
\paragraph{IS2RE without Node-Level Auxiliary Task.}
We use hyper-parameters similar to those for QM9 dataset and summarize in Table~\ref{appendix:tab:oc20}.
For ablation study in Sec.~\ref{subsec:ablation_study}, we use a smaller learning rate $1.5 \times 10 ^{-4}$ for DP attention as this improves the performance.
The detailed description of architectural hyper-parameters can be found in Sec.~\ref{appendix:subsec:equiformer_architecture}. 

%The architecture of Equiformer is the same as that for QM9 except that we use $L_{max} = 1$ and increase numbers of channels.
%Please refer to \todo{appendix} for further details.
%We apply dropout~\cite{dropout} with probability $0.2$ to attention weights. 
%We train models for $20$ epochs with AdamW optimizer~\cite{adamw}, weight decay $1 \times 10^{-3}$, batch size $32$ and cosine learning rate with linear warmup, where the maximum learning rate is $2 \times 10 ^{-4}$ and warmup epoch is $2$.



\paragraph{IS2RE with IS2RS Node-Level Auxiliary Task.}
We increase the number of Transformer blocks to $18$ as deeper networks can benefit more from IS2RS node-level auxiliary task~\citep{noisy_nodes}.
We follow the same hyper-parameters in Table~\ref{appendix:tab:oc20} except that we increase maximum learning rate to $5 \times 10^{-4}$ and set $d_{feature}$ to $[(512, 0), (256, 1)]$.
% ===============================
%   Add these back in the future
% ===============================
%Additionally, we use stochastic depth with probability $0.05$~\cite{drop_path}.
Inspired by Graphormer~\citep{graphormer_3d}, we add an extra equivariant graph attention module after the last layer normalization to predict relaxed structures and use a linearly decayed weight for loss associated with IS2RS, which starts at $15$ and decays to $1$.
For Noisy Nodes~\citep{noisy_nodes} data augmentation, we first interpolate between initial structure and relaxed structure and then add Gaussian noise as described by Noisy Nodes~\citep{noisy_nodes}.
When Noisy Nodes data augmentation is used, we increase the number of epochs to $40$.

We use two A6000 GPUs, each with 48GB, to train models when IS2RS is not included during training.
Training Equiformer and $E(3)$-Equiformer in Table~\ref{appendix:tab:e3_oc20} takes about $43.6$ and $58.3$ hours.
Training Equiformer with linear messages (indicated by Index $2$ in Table~\ref{tab:oc20_ablation}) and Equiformer with linear messages and dot product attention (indicated by Index $3$ in Table~\ref{tab:oc20_ablation}) takes $30.4$ hours and $33.1$ hours, respectively.
We use four A6000 GPUs to train Equiformer models when IS2RS node-level auxiliary task is adopted during training.
Training Equiformer without Noisy Nodes data augmentation takes about $3$ days and training with Noisy Nodes takes $6$ days.
We note that the proposed Equiformer in Table~\ref{tab:is2re_is2rs_testing} achieves competitive results even with much less computation.
Specifically, training ``Equiformer + Noisy Nodes'' takes about $24$ GPU-days when A6000 GPUs are used.
The training time of ``GNS + Noisy Nodes''~\citep{noisy_nodes} is $56$ TPU-days.
``Graphormer''~\citep{graphormer_3d} uses ensemble of $31$ models and requires $372$ GPU-days to train all models when A100 GPUs are used.




\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{ll}
%\cline{7-11}
\toprule[1.2pt]
Hyper-parameters & Value or description
 \\
\midrule[1.2pt]
Optimizer & AdamW \\
Learning rate scheduling & Cosine learning rate with linear warmup \\
Warmup epochs & $2$ \\
Maximum learning rate & $2 \times 10 ^{-4}$ \\
Batch size & $32$ \\
Number of epochs & $20$ \\
Weight decay & $1 \times 10 ^{-3}$\\
Dropout rate & $0.2$ \\
\midrule[0.6pt]
Cutoff radius ($\angstrom$) & $5$ \\
Number of radial basis & $128$ \\
Hidden size of radial function & $64$ \\
Number of hidden layers in radial function & $2$ \\

\midrule[0.6pt]

\multicolumn{2}{c}{Equiformer} \\
\\
Number of Transformer blocks & $6$ \\
Embedding dimension $d_{embed}$ & $[(256, 0), (128, 1)]$ \\
Spherical harmonics embedding dimension $d_{sh}$ & $[(1, 0), (1, 1)]$ \\
Number of attention heads $h$ & $8$ \\
Attention head dimension $d_{head}$ & $[(32, 0), (16, 1)]$\\
Hidden dimension in feed forward networks $d_{ffn}$ & $[(768, 0), (384, 1)]$ \\
Output feature dimension $d_{feature}$ & $[(512, 0)]$\\

\midrule[0.6pt]

\multicolumn{2}{c}{$E(3)$-Equiformer} \\
\\
Number of Transformer blocks & $6$ \\
Embedding dimension $d_{embed}$ & $[(256, 0, e), (64, 0, o), (64, 1, e), (64, 1, o)]$ \\
Spherical harmonics embedding dimension $d_{sh}$ & $[(1, 0, e), (1, 1, o)]$ \\
Number of attention heads $h$ & $8$ \\
Attention head dimension $d_{head}$ & $[(32, 0, e), (8, 0, o), (8, 1, e), (8, 1, o)]$ \\
Hidden dimension in feed forward networks $d_{ffn}$ & $[(768, 0, e), (192, 0, o), (192, 1, e), (192, 1, o)]$ \\
Output feature dimension $d_{feature}$ & $[(512, 0, e)]$\\

\bottomrule[1.2pt]
\end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Hyper-parameters for OC20 dataset under the setting of training without IS2RS auxiliary task.}
We denote $C_L$ type-$L$ vectors as $(C_L, L)$ and $C_{(L, p)}$ type-$(L, p)$ vectors as $(C_{(L, p)}, L, p)$ and use brackets to represent concatenations of vectors.
}
\label{appendix:tab:oc20}
\end{table}




\begin{table}[t]
\begin{adjustwidth}{-2.5 cm}{-2.5 cm}
\centering
\scalebox{0.65}{
\begin{tabular}{lccccc|ccccc}
%\cline{7-11}
\toprule[1.2pt]
 & \multicolumn{5}{c|}{Energy MAE (eV) $\downarrow$} & \multicolumn{5}{c}{EwT (\%) $\uparrow$} \\ 
\cmidrule[0.6pt]{2-11}
Methods & ID & OOD Ads & OOD Cat & OOD Both & Average & ID & OOD Ads & OOD Cat & OOD Both & Average \\
\midrule[1.2pt]
%CGCNN~\cite{cgcnn}$^{\dagger}$ & 0.6203 & 0.7426 & 0.6001 & 0.6708 & 0.6585 & 3.36 & 2.11 & 3.53 & 2.29 & 2.82 \\
SchNet~\citep{schnet}$^{\dagger}$ & 0.6465 & 0.7074 & 0.6475 & 0.6626 & 0.6660 & 2.96 & 2.22 & 3.03 & 2.38 & 2.65 \\
DimeNet++~\citep{dimenet_pp}$^{\dagger}$ & 0.5636 & 0.7127 & 0.5612 & 0.6492 & 0.6217 & 4.25 & 2.48 & 4.40 & 2.56 & 3.42 \\
GemNet-T~\citep{gemnet}$^{\dagger}$ & 0.5561 & 0.7342 & 0.5659 & 0.6964 & 0.6382 & 4.51 & 2.24 & 4.37 & 2.38 & 3.38 \\
SphereNet~\citep{spherenet} & 0.5632 & 0.6682 & 0.5590 & 0.6190 & 0.6024 & 4.56 & 2.70 & 4.59 & 2.70 & 3.64 \\
(S)EGNN~\citep{segnn} & 0.5497& 0.6851& 0.5519& 0.6102& 0.5992& 4.99& 2.50& 4.71& 2.88& 3.77 \\
SEGNN~\citep{segnn} & 0.5310& 0.6432& 0.5341& 0.5777& 0.5715& \textbf{5.32} & 2.80& 4.89& \textbf{3.09}& \textbf{4.03} \\
\midrule[0.6pt]
%Equiformer& 0.5093& 0.6285 & 0.5053 & 0.5556 & 0.5497 & 5.04 & 2.85 & 4.90 & 3.04 & \\
Equiformer & \textbf{0.5088} & \textbf{0.6271} & \textbf{0.5051} & \textbf{0.5545} & \textbf{0.5489} & 4.88 & \textbf{2.93} & \textbf{4.92} & 2.98 & 3.93 \\
%\midrule[0.6pt]
%Equiformer + NAT & 0.4685 & 0.6071 & 0.4746 & 0.5345 & 0.5212 & 5.83 & 3.18 & 5.88 & 3.43 & \\
\bottomrule[1.2pt]

\end{tabular}
}
\end{adjustwidth}
\vspace{-2mm}
\caption{\textbf{Results on OC20 IS2RE \underline{validation} set.} $\dagger$ denotes results reported by~\cite{spherenet}.}
\vspace{-2mm}
\label{tab:is2re_validation}
\end{table}


\subsection{Results on IS2RE Validation Set}
\label{appendix:subsec:is2re_validation}
For completeness, we report the results of Equiformer on the validation set in Table~\ref{tab:is2re_validation}.


\subsection{Comparison between $SE(3)$ and $E(3)$ Equivariance}
\label{appendix:subsec:e3_oc20}
We train two versions of Equiformers, one with $SE(3)$-equivariant features denoted as ``Equiformer'' and the other with $E(3)$-equivariant features denoted as ``$E(3)$-Equiformer'', and we compare them in Table~\ref{appendix:tab:e3_oc20}.
Including inversion improves the MAE results on ID and OOD Cat sub-splits but degrades the performance on the other sub-splits.
Overall, using $E(3)$-equivariant features results in slightly inferior performance.
We surmise the reasons are as follows. 
First, inversion might not be the key bottleneck. % due to the structures of input data in OC20 dataset, where a small molecule is always on top of a large slab.
Second, including inversion would break type-$1$ vectors into two parts, type-$(1, e)$ and type-$(1, o)$ vectors.
They are regarded as different types in equivariant linear layers and layer normalizations, and therefore, the directional information captured in these two types of vectors can only exchange in depth-wise tensor products.
Third, we mainly tune hyper-parameters for Equiformer with $SE(3)$-equivariant features, and it is possible that using $E(3)$-equivariant features would favor different hyper-parameters.

For Table~\ref{tab:is2re_validation},~\ref{tab:is2re_test},~\ref{tab:is2re_is2rs_validation}, and~\ref{tab:is2re_is2rs_testing}, we compare ``Equiformer'' with other works since most of them do not include equivariance to inversion.



\begin{table}[t]
\begin{adjustwidth}{-2.5 cm}{-2.5 cm}
\centering
\scalebox{0.625}{
\begin{tabular}{lccccc|cccccccc}
%\cline{7-11}
\toprule[1.2pt]
 & \multicolumn{5}{c|}{Energy MAE (eV) $\downarrow$} & \multicolumn{5}{c}{EwT (\%) $\uparrow$} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training time\\ (minutes/epoch) \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Number of \\parameters \end{tabular}} \\
\cmidrule[0.6pt]{2-11}
Methods & ID & OOD Ads & OOD Cat & OOD Both & Average & ID & OOD Ads & OOD Cat & OOD Both & Average \\
\midrule[1.2pt]
%Equiformer& 0.5093& 0.6285 & 0.5053 & 0.5556 & 0.5497 & 5.04 & 2.85 & 4.90 & 3.04 & \\
Equiformer & 0.5088 & 0.6271 & 0.5051 & 0.5545 &  0.5489 & 4.88 & 2.93 & 4.92 & 2.98 & 3.93 & 130.8 & 9.12M\\
$E(3)$-Equiformer & 0.5035 & 0.6385 & 0.5034 & 0.5658 & 0.5528 & 5.10 & 2.98 & 5.10 & 3.02 & 4.05 & 174.9 & 8.77M\\ % sh @ 1x0e + 1x1o

\bottomrule[1.2pt]

\end{tabular}
}
\end{adjustwidth}
\vspace{-2mm}
\caption{\textbf{Ablation study of $SE(3)$/$E(3)$ equivariance on OC20 IS2RE \underline{validation} set.}
``Equiformer'' operates on $SE(3)$-equivariant features while ``$E(3)$-Equiformer'' uses $E(3)$-equivariant features.
}
%\vspace{-2mm}
\label{appendix:tab:e3_oc20}
\end{table}


\subsection{Comparison of Training Time and Numbers of Parameters}
\label{appendix:subsec:oc20_training_time_comparison}
We compare training time and numbers of parameters between SEGNN~\citep{segnn} and Equiformer when IS2RS auxiliary task is not adopted during training and summarize the results in Table~\ref{appendix:tab:oc20_training_time}.
Equiformer achieves better results with comparable training time.
Please refer to Sec.~\ref{appendix:subsec:qm9_training_time_comparison} for a detailed discussion.

The comparison of training time when IS2RS auxiliary task is adopted can be found in Table~\ref{tab:is2re_is2rs_testing}.


\begin{table}[t]
\begin{adjustwidth}{-2.5 cm}{-2.5 cm}
\centering
\scalebox{0.625}{
\begin{tabular}{lccc}
%\cline{7-11}
\toprule[1.2pt]
Methods & Number of parameters & Training time (GPU-hours) \\
\midrule[1.2pt]

SEGNN~\citep{segnn} & 4.21M & 79 \\

\midrule[0.6pt]

Equiformer & 9.12M & 87 \\

\bottomrule[1.2pt]

\end{tabular}
}
\vspace{-2mm}
\end{adjustwidth}
\caption{\textbf{Comparison of training time and numbers of parameters for OC20 dataset.}  
%\note{Dropout rate = 0.1.}
%%%$\dagger$ denotes using different training, validation, testing data partitions. % as mentioned in SEGNN~\cite{segnn}.
%$\dagger$ denotes using different data partitions.
%$\ddagger$ denotes results from SE(3)-Transformer~\cite{se3_transformer}.
}
\label{appendix:tab:oc20_training_time}
\end{table}

\subsection{Error Distributions}
\label{appendix:subsec:error_distributions}
We plot the error distributions of different Equiformer models on different sub-splits of OC20 IS2RE validation set in Fig.~\ref{appendix:fig:oc20_error_distribution}.
For each curve, we sort the absolute errors in ascending order for better visualization and have a few observations.
First, for each sub-split, there are always easy examples, for which all models achieve significantly low errors, and hard examples, for which all models have high errors.
Second, the performance gains brought by different models are non-uniform among different sub-splits.
For example, using MLP attention and non-linear messages improves the errors on the ID sub-split but is not that helpful on the OOD Ads sub-split.
Third, when IS2RS node-level auxiliary task is not included during training, using stronger models mainly improves errors that are beyond the threshold of 0.02~eV, which is used to calculate the metric of energy within threshold (EwT).
For instance, on the OOD Both sub-split, using non-linear messages, which corresponds to red and purple curves, improves the absolute errors for the $15000$th through $20000$th examples.
%when the $x$ coordinate is between $15000$ and $20000$.
However, the improvement in MAE does not translate to that in EwT as the errors are still higher than the threshold of 0.02~eV.
This explains why using non-linear messages in Table~\ref{tab:oc20_ablation} improves MAE from $0.5657$ to $0.5545$ but results in almost the same EwT.


\begin{figure}
\begin{subfigure}{.495\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figure/val_id.pdf}
  \caption{\textbf{ID sub-split.}}
  \vspace{6mm}
  \label{appendix:fig:oc20_val_id}
\end{subfigure}
\begin{subfigure}{.495\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figure/val_ood_ads.pdf}
  \caption{\textbf{OOD Ads sub-split.}}
  \vspace{6mm}
  \label{appendix:fig:oc20_val_ood_ads}
\end{subfigure}
\begin{subfigure}{.495\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figure/val_ood_cat.pdf}
  \caption{\textbf{OOD Cat sub-split.}}
  \label{appendix:fig:oc20_val_ood_ads}
\end{subfigure}
\begin{subfigure}{.495\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figure/val_ood_both.pdf}
  \caption{\textbf{OOD Both sub-split.}}
  \label{appendix:fig:oc20_val_ood_ads}
\end{subfigure}
\vspace{4mm}
\caption{\textbf{Error distributions of different Equiformer models on different sub-splits of OC20 IS2RE validation set.} 
%\todo{Examples sorted by error.}
%\todo{Colors of the curves.}
}
\label{appendix:fig:oc20_error_distribution}
\end{figure}

% plot_color_gradients('Perceptually Uniform Sequential',
%                     ['viridis', 'plasma', 'inferno', 'magma', 'cividis'])





==> content/8_7_limitations.tex <==
\section{Limitations}
\label{appendix:sec:limitations}


We discuss several limitations of the proposed Equiformer and equivariant graph attention below.

First, Equiformer is based on irreducible representations (irreps) and therefore can inherit the limitations common to all equivariant networks based on irreps and the library \texttt{e3nn}~\citep{e3nn}.
For example, using higher degrees $L$ can result in larger features and using tensor products can be compute-intensive. 
Part of the reasons that tensor products can be computationally expensive are that the kernels have not been heavily optimized and customized as other operations in common libraries like PyTorch~\citep{pytorch}. 
But this is the issue related to software, not the design of networks. 
While tensor products of irreps naively do not scale well, if all possible interactions and paths are considered, some paths in tensor products can also be pruned for computational efficiency. 
We leave these potential efficiency gains to future work and in this work focus on general equivariant attention if all possible paths up to $L_{max}$ in tensor products are allowed.

Second,  the improvement of the proposed equivariant graph attention can depend on tasks and datasets. For QM9, MLP attention improves not significantly upon dot product attention as shown in Table~\ref{tab:qm9_ablation}. 
We surmise that this is because QM9 contains less atoms and less diverse atom types and therefore linear attention is enough. For OC20, MLP attention clearly improves upon dot product attention as shown in Table~\ref{tab:oc20_ablation}. Non-linear messages improve upon linear ones for the two datasets.

Third, equivariant graph attention requires more computation than typical graph convolution. 
It includes one softmax operation and thus requires one additional sum aggregation compared to typical message passing. For non-linear message passing, it increases the number of tensor products from one to two and requires more computation. 
We note that if there is a constraint on training budget, using stronger attention (i.e., MLP attention and non-linear messages) would not always be optimal because for some tasks or datasets, the improvement is not that significant and using stronger attention can slow down training. 

%For example, for the task of $C_\nu$ on QM9, using linear (index 2) or non-linear messages (index 1) results in the same performance as shown in Table~\ref{tab:qm9_ablation}.
%However, non-linear messages increase the training time of one epoch from 6.6 minutes to 11 minutes.
%}

Fourth, the proposed attention has complexity proportional to the products of numbers of channels and numbers of edges since the the attention is restricted to local neighborhoods. 
In the context of 3D atomistic graphs, the complexity is the same as that of messages and graph convolutions.
However, in other domains like computer vision, the memory complexity of convolution is proportional to the number of pixels or nodes, not that of edges. 
Therefore, it would require further modifications in order to use the proposed attention in other domains.

